Comparative Study of Approximate Multipliers

Approximate multipliers are widely being advocated for energy-efficient computing in applications that exhibit an inherent tolerance to inaccuracy. However, the inclusion of accuracy as a key design parameter, besides the performance, area and power, makes the identification of the most suitable approximate multiplier quite challenging. In this paper, we identify three major decision making factors for the selection of an approximate multipliers circuit: (1) the type of approximate full adder (FA) used to construct the multiplier, (2) the architecture, i.e., array or tree, of the multiplier and (3) the placement of sub-modules of approximate and exact multipliers in the main multiplier module. Based on these factors, we explored the design space for circuit level implementations of approximate multipliers. We used circuit level implementations of some of the most widely used approximate full adders, i.e., approximate mirror adders, XOR/XNOR based approximate full adders and Inexact adder cell. These FA cells are then used to develop circuits for the approximate high order compressors as building blocks for 8x8 array and tree multipliers. We then develop various implementations of higher bit multipliers by using a combination of exact and inaccurate 8x8 multiplier cells. All these implementations have been done using the Cadence's Spectre tool with the TSMC65nm technology. The design space of these multipliers is explored based on their power, area, delay and error and the best approximate multiplier designs are identified. The report also presents the validation of our results using an image blending application. An open source library of implemented cells and multiplier circuits are available online.

==> Arxiv-Online-Comparative-TR uploaded/Application.tex <==
\section{\textbf{Application}} \label{sec:application}

%We evaluate and compare the accuracy of the built approximate multipliers based on an image blending application, where two images are multiplied pixel-by-pixel.

While in previous sections, we used Cadence Spectre to build the circuits and evaluate their area, performance and power consumption. In this section, for experimentation purposes, we evaluate and compare the accuracy of the built approximate multipliers based on an image blending application, where two images are multiplied pixel-by-pixel as shown in Figure \ref{fig:blinding}. Here, we use MATLAB to evaluate error metrics for image processing. To this end, we have modeled the same approximate multiplier circuit architectures in MATLAB and run exhaustive simulation.
%The circuits have been implemented in MATLAB and an exhaustive simulation was conducted. Cadence have been used to build the circuits and evaluate their area, performance and power consumption, i.e, EDIF file is used for netlist exchange. However, evaluation of error metrics and image processing is suitable using MATLAB .

\begin{figure}[!t]
\centering
\includegraphics[width=14cm, height=5cm]{blinding.png}
\caption{Image blinding}
\label{fig:blinding}
\end{figure}

The signal to noise ratio (SNR) is used to measure the image quality. Figure \ref{fig:PDP_SNR} shows a comparison of the SNR and the percentage of PDP reduction for different approximate multipliers. Designs on the bottom left corner, have the highest PDP reduction and the best quality (high SNR). Generally, all multiplier designs have an acceptable SNR (acceptable quality). However, there exist some designs, e.g., \textit{16EIn3}, \textit{16CEX2} and \textit{16CX2X2}, with PDP greater than the exact design. The library of implemented cells and multiplier circuits, and the results of the image blending application can be found at
\textit{https://sourceforge.net/projects/approximatemultiplier}.


%\includegraphics[width=9cm]{PDP_SNR44.jpg}
\begin{figure}[h]
\centering
\includegraphics[width=1.0\textwidth, height=6cm]{PSNR-P2.png}
\caption{\%PDP Reduction and SNR of Multipliers}
\label{fig:PDP_SNR}
\end{figure}

%\section{\textbf{\color{red}Comparison with Previous Work}} 

%Error rate (ER) indicates the probability of producing incorrect result. However, it does not indicate error significance. Therefore, NMED which is the normalization of MED by the maximum output of the correct design, is used to compare designs of different sizes.
%We compared our work with a 24 different designs of approximate multipliers, reported in \cite{Jiang}. Regarding ER, 92\% of their designs (22 designs out of 24) were found to have ER close to 100\% while only 80\% (24 out of 30) of our proposed designs have high ER. Regarding NMED, almost all our designs (26 out of 30) have a value less than 10\textsuperscript{-5}, which is the minimum value reported by the 24 approximate designs in \cite{Jiang}. Comparing the PDP reduction, most of the designs in \cite{Jiang} have a high PDP reduction because they are based on truncation and a high degree of approximation. However, our designs are superior in PDP reduction for designs with low degree of approximation.

%Most of the designs in \cite{Jiang} rely on approximation on partial product generation, truncation of partial product tree and reduction of carry propagation path. However, our designs generate exact partial products, without tree truncation nor reduction of carry path propagation.

%Comparing Power, delay and PDP as absolute values cannot be considered as a fair comparison because of the involvement of different process technology (our work based on TSMC65nm and the work in \cite{Jiang} is based on STM CMOS 28nm). 
%Comparing the PDP reduction, most of the designs in \cite{Jiang} have a high PDP reduction because they are based on truncation and a high degree of approximation compared to our designs. However, our designs have a competitive PDP reduction with the designs, which have low degree of approximation. %Based on our results, increasing the degree of approximation of our designs, provides a higher PDP reduction, and thus making these designs useful for the applications  that have a higher tolerance for accuracy. %Our work and \cite{Jiang} shows that image sharpening application based on approximate multipliers with low accuracy provides a high PDP reduction and give results with high quality expressed as high PSNR, designs with high accuracy provides a low PDP reduction and give results with low quality expressed as low PSNR}.


==> Arxiv-Online-Comparative-TR uploaded/ApproximateFAs.tex <==

\section{\textbf{Approximate FAs and Compressors}} \label{sec:ApproxFA}


Approximate n-bit binary adders can be designed by modifying the carry generation and propagation of the addition process by using several overlapping sub-adders to reduce latency. Some examples include speculative \cite{speculative}, segmented \cite{segmented} and carry select adders \cite{CSA}. However, these designs involve several overlapping sub-adders, which makes them unsuitable to build energy efficient circuits. Low power approximate binary adders are generally constructed by replacing the accurate FAs with approximate FAs. We consider five approximate mirror adders (AMA1, AMA2, AMA3, AMA4 and AMA5) \cite{Vaibhav}, three approximate XOR/XNOR based full adders (AXA1, AXA2 and AXA3) \cite{XORFA} and three inexact adder cells (InXA1, InXA2 and InXA3) \cite{InXA}.

Table \ref{tab:FA} shows the truth tables of the 11 considered approximate FAs, and their characteristics including Size (A), Power consumption (P), Delay (D), number of Erroneous outputs (E), which indicates the likelihood of at least one output (Cout or Sum) being wrong, and PDP. \textit{All approximate FAs are Pareto-points}, i.e., they provide less area and power consumption compared to the exact design at the cost of compromising accuracy \cite{Pareto}. Some of the FA designs have an enhanced performance (reduced delay), while other designs have degraded performance due to the internal structure and node capacitance. In \cite{Rehman}, AMA5 is considered as a \textit{wire} with zero area and zero power consumption. However, this is unrealistic as the output of AMA5 has to drive other signals. Thus, we used two buffers instead of two wires to design it.
%
%\begin{figure*}[th]
%\includegraphics[width=16cm]{FullAdder.png}
%\caption{Truth Tables and Characteristics (Size, Power, Delay, \# Error Cases and PDP) of Different Approximate FAs )}
%\label{fig:FA}
%\end{figure*}


\begin{table*}[th!]
  \centering
  \caption{Truth Tables of Different Approximate FAs and Comparison of their Characteristics}
  %\scalebox{0.7}{  
\resizebox{0.99\textwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|cc|}
    \toprule
    \multicolumn{3}{|c|}{\textbf{Inputs}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .294,  .675,  .776} \textbf{Exact FA (E)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .314} \textbf{AMA1 (M1)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .314} \textbf{AMA2 (M2)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .314} \textbf{AMA3 (M3)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .314} \textbf{AMA4 (M4)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .314} \textbf{AMA5 (M4)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .941} \textbf{AXA1 (X1)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .941} \textbf{AXA2 (X2)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 0,  .69,  .941} \textbf{AXA3 (X3)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  .753,  0} \textbf{InXA1 (In1)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  .753,  0} \textbf{InXA2 (In2)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  .753,  0} \textbf{InXA3 (In3)}} \\
    \midrule
    \textbf{A} & \textbf{B} & \textbf{Cin} & \cellcolor[rgb]{ .573,  .804,  .863} \textbf{Sum} & \cellcolor[rgb]{ .573,  .804,  .863} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{Sum}} & \cellcolor[rgb]{ .847,  .894,  .737} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{Sum}} & \cellcolor[rgb]{ .847,  .894,  .737} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{Sum}} & \cellcolor[rgb]{ .847,  .894,  .737} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{Sum}} & \cellcolor[rgb]{ .847,  .894,  .737} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{Sum}} & \cellcolor[rgb]{ .847,  .894,  .737} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{Sum}} & \cellcolor[rgb]{ .773,  .851,  .945} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{Sum}} & \cellcolor[rgb]{ .773,  .851,  .945} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{Sum}} & \cellcolor[rgb]{ .773,  .851,  .945} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{Sum}} & \cellcolor[rgb]{ .988,  .835,  .706} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{Sum}} & \cellcolor[rgb]{ .988,  .835,  .706} \textbf{Cout} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{Sum}} & \cellcolor[rgb]{ .988,  .835,  .706} \textbf{Cout} \\
    \midrule
    0  & 0 & 0  & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{0} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{0} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{0} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} \\
    \midrule
    0  & 0  & 1  & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0 \\
    \midrule
    0  & 1  & 0  & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0 \\
    \midrule
    0  & 1  & 1  & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{0} & 1 \\
    \midrule
    1  & 0  & 0  & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{1} & 0     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \multicolumn{1}{c|}{1} & 0 \\
    \midrule
    1  & 0  & 1  & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{0} & 1 \\
    \midrule
    1  & 1  & 0  & \cellcolor[rgb]{ .851,  .851,  .851} 0 & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{1}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{0}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 0} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{0} & 1 \\
    \midrule
    1  & 1  & 1  & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{1} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \cellcolor[rgb]{ .851,  .851,  .851} \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{1} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{1} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{1} & 1     & \multicolumn{1}{c|}{\cellcolor[rgb]{ .851,  .851,  .851} 1} & \cellcolor[rgb]{ .851,  .851,  .851} 1 & \multicolumn{1}{c|}{\textcolor[rgb]{ 1,  0,  0}{\textbf{0}}} & \textcolor[rgb]{ 1,  0,  0}{\textbf{1}} \\
    \midrule
    \rowcolor[rgb]{ .902,  .722,  .718} \multicolumn{3}{|c|}{\textbf{Size}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  1,  1} \textbf{28}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .769,  .843,  .608} \textbf{20}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .769,  .843,  .608} \textbf{14}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .769,  .843,  .608} \textbf{11}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .769,  .843,  .608} \textbf{15}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .769,  .843,  .608} \textbf{8}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{8}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{6}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{8}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{6}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{8}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{6}} \\
    \midrule
    \rowcolor[rgb]{ .902,  .722,  .718} \multicolumn{3}{|c|}{\textbf{Power (nw)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  1,  1} \textbf{763.3}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{612}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{561.1}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{558.1}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{587.1}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{412.1}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{676.2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{358.7}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{396.5}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{410}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{355.1}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{648}} \\
    \midrule
    \rowcolor[rgb]{ .902,  .722,  .718} \multicolumn{3}{|c|}{\textbf{Delay (ps)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  1,  1} \textbf{244}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{195}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{366}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{360}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{196}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{150}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{1155}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{838}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{1467}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{740}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{832}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{767}} \\
    \midrule
    \rowcolor[rgb]{ .902,  .722,  .718} \multicolumn{3}{|c|}{\textbf{\# of Error Cases}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  1,  1} \textbf{0}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{3}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{3}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} \textbf{4}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{4}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{4}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .553,  .706,  .886} \textbf{2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{2}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .992,  .914,  .851} \textbf{2}} \\
    \midrule
    \rowcolor[rgb]{ .902,  .722,  .718} \multicolumn{3}{|c|}{\textbf{PDP (fJ)}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ 1,  1,  1} \textbf{186.25}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{119.34}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{205.36}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{200.92}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{115.07}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .847,  .894,  .737} \textbf{61.82}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{781}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{300.59}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .773,  .851,  .945} \textbf{582}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{303.4}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{295.44}} & \multicolumn{2}{c|}{\cellcolor[rgb]{ .988,  .835,  .706} \textbf{753.5}} \\
    \bottomrule
    \end{tabular} }
  \label{tab:FA}
\end{table*}


\begin{figure}[!t]
\centering
\includegraphics[width=1.0\textwidth, height=5cm]{P_D_FA.png}
\caption{Power Consumption and Delay of Approximate FAs}
\label{fig:Power_Delay_FA}
\end{figure}



%\begin{figure}[!h]
%\centering
%\includegraphics[width=11cm]{FA_PDP.png}
%\caption{PDP of Approximate FAs}
%\label{fig:PDP_FA}
%\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=1.0\textwidth, height=5cm]{PDP1.png}
\caption{Power-Delay-Product of Approximate FAs}
\label{fig:PDP_FA}
\end{figure}

\begin{figure}[!t]
\centering
%\includegraphics[width=1.0\textwidth, height=6cm]{A_ER_FA.png}
\includegraphics[width=1.0\textwidth, height=5cm]{A_ER_FA.png}
\caption{Size and Number of erroneous outputs (ER) of Approximate FAs}
\label{fig:Area_ER_FA}
\end{figure}


% with a reduced internal node capacitance
%\begin{table}[h]
%\caption{Power, Delay, and PDP of Approximate FAs}
%%\begin{center}
%\resizebox{\columnwidth}{!} {%
%\begin{tabular}{cccc||cccc}
%\hline
%\textbf{FA Type}&\textbf{Power($\mu$w})& \textbf{Delay(ps)} & \textbf{PDP(fj)} &\textbf{FA Type} &\textbf{Power($\mu$w)}& \textbf{Delay(ps)} &  \textbf{PDP(fj)} \\ \hline \hline			
%\textbf{Exact MA}&763.3	&244&186.25 &\textbf{AXA1}&676.2&3155&2133.41 \\ \hline
%\textbf{AMA1}&612	&\cellcolor{yellow}\textbf{195}&119.34 & \textbf{AXA2}&\cellcolor{yellow}\textbf{358.7}&838&300.59 \\  \hline
%\textbf{AMA2}&561.1	&366&205.36 & \textbf{AXA3}&396.5&3600&1427.4 \\  \hline
%\textbf{AMA3}&558.1	&360&200.92 &\textbf{InXA1}&410	&740&303.4 	\\  \hline
%\textbf{AMA4}&587.1	&\cellcolor{yellow}\textbf{196}&115.07 & \textbf{InXA2}&\cellcolor{yellow}\textbf{355.1}&832&295.44 \\  \hline
%\textbf{AMA5}&412.1	&\cellcolor{yellow}\textbf{150}&\cellcolor{yellow}\textbf{61.82}  & \textbf{InXA3}&982.4&767&753.5  \\   \hline
%\end{tabular} } 
%\label{table:FAs}
%\end{table}


%Figure \ref{fig:Area_ER_FA} depicts the size of FAs in terms of the number of transistors, and the error rate for both \textit{Cout} and \textit{Sum}.

Figure \ref{fig:Power_Delay_FA} shows the power consumption and delay of individual approximate FAs, where all FAs exhibit a reduced power consumption. But, only the mirror adder based FAs have a reduced delay due to their internal structure. InXA2 and AXA2 have the minimal power consumption with 53\% reduction compared to the exact mirror adder (MA). Also, InXA1 and AXA3 have close-to-minimal power consumption. Since AMA5 is composed of only two buffers, it has the lowest delay while AXA3 has the highest delay due to the threshold voltage drop of the pass transistors. AMA1 and AMA4 both have a close-to-minimal delay. PDP which is a figure of merit correlated with the energy efficiency of a digital design, is shown in Figure \ref{fig:PDP_FA} for the FAs. Mirror adder based designs have a low PDP values. AMA5 and AXA1 exhibit the lowest and highest PDP, respectively. 

Figure \ref{fig:Area_ER_FA} shows the number of transistors for each FA, as well the number of erronous outputs. AXA2, InXA1 and InXA3 consist of 6 transistors each, and thus have a 78.6\% area reduction compared to the exact MA. AMA5, AXA1, AXA3 and InXA2 all have 8 transistors. AMA5, AXA1 and AXA2 have 4 erroneous outputs. AMA3 and AMA4 have 3 erroneous outputs, and the remaining 6 designs have 2 erroneous outputs. Our results are consistent with the findings reported in \cite{Vaibhav}\cite{XORFA}\cite{InXA}.

%AXA1 shows the highest ER for both \textit{Sum} and \textit{Cout}. AMA5, AXA2 and InXA2 have the highest ER for \textit{Sum}.



Assuming that the characteristics of approximate FAs are linearly applied to approximate arithmetic circuits (adders and multipliers), there is no single approximate FA, which is superior in all aspects. Therefore, we propose to use a \textit{fitness function} to evaluate the designs based on its design metrics.
\begin{equation}
Fitness = \textit{C1}*A + \textit{C2}*P +  \textit{C3}*D + \textit{C4}*E + \textit{C5}*PDP 
\label{eq:fitness}
\end{equation} where \textit{C1}, \textit{C2}, \textit{C3}, \textit{C4} and \textit{C5} are application-dependent design coefficients within the range [0,1] which provide weights to specific design metrics for a specific application, e.g., E equals zero for the exact designs where approximation is not allowed, and P is small for low power designs depending of application error-resiliency. The fitness of the approximate circuit depends on the application resiliency and input data distribution. \textit{A minimal fitness value is preferred since the goal is to minimize A, P, D and E}. For the remainder of this work, we use all 11 Pareto-design approximate FAs as elementary building cells to construct approximate array multipliers. 

\begin{figure}[!t]
\centering
\includegraphics[width=8cm , height=6cm]{8to4Compressor1.png}
\caption{8-to-4 Compressor Design}
\label{fig:8to4}
\end{figure}

Higher-order compressors, e.g., 5-to-3 (which compresses
five partial product bits into three) and 8-to-4 (which compresses eight partial product bits into four) \cite{M2}, allow us to construct high speed tree multipliers. Therefore, we also developed approximate FA based compressors, e.g., a 8-to-4 binary compressor is depicted in Figure \ref{fig:8to4}, for evaluation purposes. Table \ref{tab:Compressor} shows the power consumption and area for different approximate compressors implemented using approximate FAs. The area for approximate compressors exhibits a linear relationship with the area of FAs. However, it looks difficult to obtain a closed-form analytical expression for the power consumption. Few designs have a larger power consumption compared to the exact one, and this behavior needs more investigation. For that, and as a future work, we plan to use several approximate compressors with different approximation degrees in order to cover a larger design space.
Considering all options, the total combination of compressor settings grows exponentially O( (\# of FA designs)\textsuperscript{\# of FAs in compressor}) = O (11)\textsuperscript{4} = 14641 in our case. Therefore, to show the effectiveness of designing approximate compressors based on approximate FAs, we chose four FAs only. These FAs have superior designs metrics. The best approximate FA in terms of delay and PDP was \textit{AMA5}, and in terms of power and area was \textit{AXA2}. Also, the best FA with low error rate was \textit{InXA1}. \textit{AMA3} has moderate characteristics regarding area, power, delay, and number of errors. These selected FAs are used to design approximate high-order compressors, which in turn can be used for designing approximate tree multipliers. \textit{However, these selected compressors are not guaranteed to be the optimal ones. But, they exhibit some improvements compared to the exact designs.}




\begin{table}[!t]
  \centering
  \caption{Power Consumption and Area for Different Approximate Compressors based on Different Approximate FAs}
  \resizebox{0.99\textwidth}{!} {
    \begin{tabular}{|c|c|c|c|c|c|c|r|c|c|c|c|c|c|c|}
\cmidrule{2-7}\cmidrule{10-15}    \multicolumn{1}{r|}{} & \multicolumn{6}{c|}{Power Consumption ($\mu$w)for Different Compressors} & \multicolumn{1}{r}{} &       & \multicolumn{6}{c|}{Area (number of transistors)for Different Compressors} \\
\cmidrule{2-7}\cmidrule{10-15}    \multicolumn{1}{r|}{} & \multicolumn{6}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} Compressor Type} & \multicolumn{1}{r}{} &       & \multicolumn{6}{c|}{\cellcolor[rgb]{ .573,  .816,  .314} Compressor Type} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{FA Type} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{3-2} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{4-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{5-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{6-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{7-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{8-4} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{FA Type} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{3-2} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{4-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{5-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{6-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{7-3} & \cellcolor[rgb]{ .573,  .816,  .314} \textbf{8-4} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{Exact} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.562} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.469} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.659} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.466} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.355} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{2.198} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{Exact} & \cellcolor[rgb]{ 1,  1,  1} \textbf{28} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{56} & \cellcolor[rgb]{ 1,  1,  1} \textbf{70} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{98} & \cellcolor[rgb]{ 1,  1,  1} \textbf{112} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{154} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{M1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.5474} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.9696} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.494} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.9258} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.138} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.65} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{M1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{20} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{48} & \cellcolor[rgb]{ 1,  1,  1} \textbf{54} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{74} & \cellcolor[rgb]{ 1,  1,  1} \textbf{80} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{122} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{M2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4525} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.224} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.189} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.536}} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.321} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.609} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{M2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{14} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{42} & \cellcolor[rgb]{ 1,  1,  1} \textbf{42} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{56} & \cellcolor[rgb]{ 1,  1,  1} \textbf{56} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{98} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{M3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4489} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.6813} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.378} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.073} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.6157} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.9114} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{M3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{11} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{39} & \cellcolor[rgb]{ 1,  1,  1} \textbf{36} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{47} & \cellcolor[rgb]{ 1,  1,  1} \textbf{44} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{86} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{M4} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.5228} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.9988} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.176} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.183} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.037} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.449} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{M4} & \cellcolor[rgb]{ 1,  1,  1} \textbf{15} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{43} & \cellcolor[rgb]{ 1,  1,  1} \textbf{44} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{59} & \cellcolor[rgb]{ 1,  1,  1} \textbf{60} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{102} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{M5} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4802} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.9333} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.199} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.023} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.8753} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.791} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{M5} & \cellcolor[rgb]{ 1,  1,  1} \textbf{8} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{36} & \cellcolor[rgb]{ 1,  1,  1} \textbf{30} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{38} & \cellcolor[rgb]{ 1,  1,  1} \textbf{32} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{74} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{X1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4511} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.586}} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.128} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.562}} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.521}} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{2.142} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{X1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{8} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{36} & \cellcolor[rgb]{ 1,  1,  1} \textbf{30} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{38} & \cellcolor[rgb]{ 1,  1,  1} \textbf{32} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{74} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{X2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4584} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.296} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.563} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.8141} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.7489} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{2.77}} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{X2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{6} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{34} & \cellcolor[rgb]{ 1,  1,  1} \textbf{26} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{32} & \cellcolor[rgb]{ 1,  1,  1} \textbf{24} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{66} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{X3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.3544} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.349} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.429} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.231} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.4742} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{2.316}} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{X3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{8} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{36} & \cellcolor[rgb]{ 1,  1,  1} \textbf{30} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{38} & \cellcolor[rgb]{ 1,  1,  1} \textbf{32} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{74} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{In1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.1823} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.569}} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.9423} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.4842} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.296} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{2.413}} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{In1} & \cellcolor[rgb]{ 1,  1,  1} \textbf{6} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{34} & \cellcolor[rgb]{ 1,  1,  1} \textbf{26} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{32} & \cellcolor[rgb]{ 1,  1,  1} \textbf{24} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{66} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{In2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.5018} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.324} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{2.114}} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.3441} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.8087} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{3.844}} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{In2} & \cellcolor[rgb]{ 1,  1,  1} \textbf{8} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{36} & \cellcolor[rgb]{ 1,  1,  1} \textbf{30} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{38} & \cellcolor[rgb]{ 1,  1,  1} \textbf{32} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{74} \\
\cmidrule{1-7}\cmidrule{9-15}    \rowcolor[rgb]{ 1,  1,  0} \textbf{In3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{0.5504} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{1.345} & \cellcolor[rgb]{ 1,  1,  1} \textbf{1.234} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{0.7866} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{1.636}} & \cellcolor[rgb]{ 1,  .78,  .808} \textcolor[rgb]{ .612,  0,  .024}{\textbf{5.27}} & \cellcolor[rgb]{ 1,  1,  1}  & \textbf{In3} & \cellcolor[rgb]{ 1,  1,  1} \textbf{6} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{34} & \cellcolor[rgb]{ 1,  1,  1} \textbf{26} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{32} & \cellcolor[rgb]{ 1,  1,  1} \textbf{24} & \cellcolor[rgb]{ .851,  .851,  .851} \textbf{66} \\
\cmidrule{1-7}\cmidrule{9-15}    
\end{tabular}%
}
  \label{tab:Compressor}%
\end{table}%




%It can be noted from the above results that all approximate FAs exhibit an improved delay, area and power compared to the exact FA, but these benefits have been acquired at the cost of some accuracy loss. However, there is no single approximate FA, which is superior in all aspects. Therefore in this work, we use all these 11 approximate FAs as elementary building cells to construct approximate array multipliers. Also, we chose the best approximate FAs in terms of delay (\textit{AMA5}), power and area (\textit{AXA2}), low ER for both \textit{Sum} and \textit{Cout} (\textit{InXA1}), and moderate characteristics regarding area, power, delay, and ER (\textit{AMA3}), to design approximate high-order compressors, which in turn can be used for designing approximate tree multipliers. 

==> Arxiv-Online-Comparative-TR uploaded/BasicBlock.tex <==

\section{\textbf{Multiplier Basic Blocks}} \label{sec:8X8}

In this section, we use the approximate FAs and compressors, described above, to design 8x8 array and tree based multipliers, respectively. These 8x8 approximate multipliers will act as our basic blocks for designing higher-order multipliers, i.e., 32x32 and 64x64, as it will be discussed in Section \ref{sec:MainModule}.

\subsection{\textbf{8x8 Array Multiplier}}  \label{sec:Array8}
 An n-bit array multiplier \cite{rabaey} is composed of \textit{n\textsuperscript{2}} AND gates for partial products generation, and \textit{n-1} n-bit adders for partial products accumulation. The design space of an \textit{n}x\textit{n} approximate array multiplier is quite huge, since it depends on the type of FA used in the array, and the \textit{number} of approximate FAs (from 0 to \textit{n}) used in the n-bit adder. Considering all options, the total combination of multiplier settings grow exponentially O( (\# of FAs)\textsuperscript{MultiplierSize\textsuperscript{2}}) = O ((11)\textsuperscript{n\textsuperscript{2}}) = (11)\textsuperscript{64} in our case.
%To reduce the design space, we have chosen to design each basic multiplier module (8x8 approximate array multiplier) using only one type of approximate FA (11 options)

We have used all 11 Pareto approximate FAs, described in Section \ref{sec:ApproxFA}, to construct 8x8 approximate array multipliers, based on only one FA type per design to avoid the exponential growth of the design space. Regarding the degree of approximation, we have used two options: i) all FAs are approximate, and ii) FAs that contribute to the least significant 50\% of the resultant bits are approximated to maintain acceptable accuracy as recommended by \cite{Vaibhav} \cite{Reddy} \cite{Shao}. Thus, we have designed, evaluated and compared 22 different options for building 8x8 approximate array multipliers as shown in Table \ref{table:8X8Array}, using the TSMC65nm technology. The type of the multiplier in Table \ref{table:8X8Array} consists of two parts, i.e., the name of the adder used for the most significant and least significant part. For example, in EM1, the most significant part is based on an exact (E) adder and the least significant part is based on the mirror adder 1 (M1). 
  
 
%However, for our error-oriented approximate designs, another approximation degree (from 1 to \textit{2n}) can be specified based on the maximum error allowed for each application using Algorithm \ref{alg:ApproximationDegree}. \textcolor{red}{The algorithm accepts the exact design, set of proposed approximate designs with different degrees of approximation (from 1 to 2n) and a design metric to specify the maximum degree of approximation (for error-oriented designs E\textsubscript{Max} is used and for area-oriented design A\textsubscript{Max} is used). The algorithm  is iterative (Line 2 - 6) and performs success error evaluation until the imposed target error constraint is violated. The algorithm proceeds to the next iteration if the approximate circuit error is less than the specified error constrain, otherwise the last acceptable approximation degree with its corresponding design is returned as the output (Line 7).}
 

 
 
%\begin{table}[!t]
%\centering
% \caption{8x8 Approximate Array Multiplier}
% %\resizebox{\columnwidth}{!}{%
% \scalebox{0.85}{   
%   \begin{tabular}{|c|c|c|c|c|c|} \hline
%\textbf{Type} & \textbf{ER} &\textbf{NMED} &\textbf{Delay}(PS) &	\textbf{POWER}($\mu$W)&	\textbf{SIZE}  \\   \hline \hline
%\textbf{EE}	&0	&0	&527&31.41	&1456\\ \hline
%\textbf{EM1}&9.70x10\textsuperscript{-1}&3.93x10\textsuperscript{-3}&	527&24.17&1288\\ \hline
%\textbf{M1M1}&9.96x10\textsuperscript{-1}&2.05x10\textsuperscript{-1}&865&14.75&1072\\ \hline
%\textbf{EM2}&9.90x10\textsuperscript{-1}&3.52x10\textsuperscript{-3}&557&22.97&	1162\\ \hline
%\textbf{M2M2}&1.00 	&2.58x10\textsuperscript{-1}&	600	&14.4&	784\\ \hline
%\textbf{EM3}&9.99 x10\textsuperscript{-1}&7.26x10\textsuperscript{-3}&	605	&24.95&1099\\ \hline
%\textbf{M3M3}&1.00	&2.64x10\textsuperscript{-1}&598	&15.31&	640\\ \hline
%\textbf{EM4}&9.70x10\textsuperscript{-1}&	\cellcolor{yellow}\textbf{1.71x10\textsuperscript{-3}}&573&	21.85&	1183\\ \hline
%\textbf{M4M4}&9.96x10\textsuperscript{-1}&	9.86x10\textsuperscript{-2}&\textbf{313}	&\cellcolor{yellow}\textbf{11.17}&	832\\ \hline
%\textbf{EM5}&9.30x10\textsuperscript{-1}&\cellcolor{yellow}\textbf{1.56x10\textsuperscript{-3}}&573&22.15&	1036\\ \hline
%\textbf{M5M5}&9.90x10\textsuperscript{-3}	&1.27x10\textsuperscript{-1}&\cellcolor{yellow}\textbf{250}	&\cellcolor{yellow}\textbf{10.69}&	496\\ \hline  \hline
%\textbf{EX1}&9.71x10\textsuperscript{-3}	&3.21x10\textsuperscript{-3}&546	&31.86&	1036\\ \hline
%\textbf{X1X1}&9.96x10\textsuperscript{-3}&	1.61x10\textsuperscript{-1}&558	&21.33	&496\\ \hline
%\textbf{EX2}&1.00&	2.89x10\textsuperscript{-3}&569&23.38&	994\\ \hline
%\textbf{X2X2}&1.00&	2.31x10\textsuperscript{-1}&\cellcolor{yellow}\textbf{250}	&13.91	&\cellcolor{yellow}\textbf{400}\\ \hline
%\textbf{EX3}&\cellcolor{yellow}\textbf{6.15x10\textsuperscript{-1}}	&5.35x10\textsuperscript{-3}&536&	25.54&	1036\\ \hline
%\textbf{X3X3}&9.96x10\textsuperscript{-1}&	2.50x10\textsuperscript{-1}&\cellcolor{yellow}\textbf{197}&	15.06&	496\\ \hline  \hline
%\textbf{EIn1}&\cellcolor{yellow}\textbf{6.15x10\textsuperscript{-1}}&4.91x10\textsuperscript{-3}&517&26.07&994\\ \hline
%\textbf{In1In1}&8.54x10\textsuperscript{-1}&	1.56x10\textsuperscript{-1}&403&14.82&	\cellcolor{yellow}\textbf{400}\\ \hline
%\textbf{EIn2}&\cellcolor{yellow}\textbf{5.84x10\textsuperscript{-1}}&\cellcolor{yellow}\textbf{2.76x10\textsuperscript{-3}}&	528	&28.79	&1036\\ \hline
%\textbf{In2In2}&8.26x10\textsuperscript{-1}&1.27x10\textsuperscript{-1}&	340	&\cellcolor{yellow}\textbf{12.56}&	496\\ \hline
%\textbf{EIn3}&9.90x10\textsuperscript{-1}&3.52x10\textsuperscript{-3}&	556	&27.96&	994\\ \hline
%\textbf{In3In3}&1.00&	2.58x10\textsuperscript{-1}&	404	&23.92&	\cellcolor{yellow}\textbf{400}\\ \hline
%\end{tabular}  }
%\label{table:8X8Array}
%\end{table}


% Table generated by Excel2LaTeX from sheet '8x8Array'
\begin{table}[!t]
  \centering
  \caption{8x8 Approximate Array Multiplier}
  \scalebox{0.7}{  
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \toprule
  %  \multirow{3}[2]{*}{\textbf{Type}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{MRED}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{MED}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{ER}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{NMED}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{Delay (ps)}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{POWER ($\mu$W)}}} & \multicolumn{1}{c|}{\multirow{3}[2]{*}{\textbf{SIZE}}} \\
  %  \multicolumn{1}{|c|}{} &       &       &       &       &       &       &  \\
   % \multicolumn{1}{|c|}{} &       &       &       &       &       &       &  \\
          \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{2.555em}|}{\textbf{Delay (ps)}} & \multicolumn{1}{p{2.78em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{2.11em}|}{\textbf{size}} \\
    \midrule
    \textbf{EE} & 00  & 00   & 00  & 00   & 527   & 31.41 & 1456 \\
    \midrule
    \textbf{EM1} & 8.55E-02 & 2.55E+02 & 9.70E-01 & 3.93E-03 & 527   & 24.17 & 1288 \\
    \midrule
    \textbf{M1M1} & 2.13E+00 & 1.33E+04 & 9.96E-01 & 2.05E-01 & 865   & 14.75 & 1072 \\
    \midrule
    \textbf{EM2} & 1.85E-01 & 2.29E+02 & 9.90E-01 & 3.52E-03 & 557   & 22.97 & 1162 \\
    \midrule
    \textbf{M2M2} & 1.73E+01 & 1.68E+04 & 1.00E+00 & 2.58E-01 & 600   & 14.4  & 784 \\
    \midrule
    \textbf{EM3} & 4.03E-01 & 4.72E+02 & 9.99E-01 & 7.26E-03 & 605   & 24.95 & 1099 \\
    \midrule
    \textbf{M3M3} & 1.25E+01 & 1.72E+04 & 1.00E+00 & 2.64E-01 & 598   & 15.31 & 640 \\
    \midrule
    \textbf{EM4} & 3.64E-02 & 1.11E+02 & 9.70E-01 & 1.71E-03 & 573   & 21.85 & 1183 \\
    \midrule
    \textbf{M4M4} & 6.11E-01 & 6.41E+03 & 9.96E-01 & 9.86E-02 & 313   & 11.17 & 832 \\
    \midrule
    \textbf{EM5} & 3.03E-02 & 1.01E+02 & 9.30E-01 & 1.56E-03 & 573   & 22.15 & 1036 \\
    \midrule
    \textbf{M5M5} & 6.76E-01 & 8.24E+03 & 9.90E-01 & 1.27E-01 & 250   & 10.69 & 496 \\
    \midrule
    \textbf{EX1} & 1.18E-01 & 2.09E+02 & 9.71E-01 & 3.21E-03 & 546   & 31.86 & 1036 \\
    \midrule
    \textbf{X1X1} & 2.84E+00 & 1.05E+04 & 9.96E-01 & 1.61E-01 & 558   & 21.33 & 496 \\
    \midrule
    \textbf{EX2} & 1.09E-01 & 1.88E+02 & 1.00E+00 & 2.89E-03 & 569   & 23.38 & 994 \\
    \midrule
    \textbf{X2X2} & 1.18E+01 & 1.51E+04 & 1.00E+00 & 2.31E-01 & 250   & 13.91 & 400 \\
    \midrule
    \textbf{EX3} & 7.96E-02 & 3.48E+02 & 6.15E-01 & 5.35E-03 & 536   & 25.54 & 1036 \\
    \midrule
    \textbf{X3X3} & 9.88E-01 & 1.63E+04 & 9.96E-01 & 2.50E-01 & 197   & 15.06 & 496 \\
    \midrule
    \textbf{EIn1} & 7.50E-02 & 3.19E+02 & 6.15E-01 & 4.91E-03 & 517   & 26.07 & 994 \\
    \midrule
    \textbf{In1In1} & 1.62E+00 & 1.02E+04 & 8.54E-01 & 1.56E-01 & 403   & 14.82 & 400 \\
    \midrule
    \textbf{EIn2} & 3.68E-02 & 1.80E+02 & 5.84E-01 & 2.76E-03 & 528   & 28.79 & 1036 \\
    \midrule
    \textbf{In2In2} & 4.63E-01 & 8.28E+03 & 8.26E-01 & 1.27E-01 & 340   & 12.56 & 496 \\
    \midrule
    \textbf{EIn3} & 1.85E-01 & 2.29E+02 & 9.90E-01 & 3.52E-03 & 556   & 27.96 & 994 \\
    \midrule
    \textbf{In3In3} & 1.73E+01 & 1.68E+04 & 1.00E+00 & 2.58E-01 & 404   & 23.92 & 400 \\
    \bottomrule
    \end{tabular}%
    }
  \label{table:8X8Array}
\end{table}%


% Table generated by Excel2LaTeX from sheet '8x8Array'
%\begin{table}[!t]
%\centering
% \caption{8x8 Approximate Array Multiplier}
% %\resizebox{\columnwidth}{!}{%
% \scalebox{0.8}{   
%    \begin{tabular}{|c|c|c|c|c|c|c|c|}
%      %  \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{4.055em}|}{\textbf{Delay (PS)}} & \multicolumn{1}{p{4.055em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{4.055em}|}{\textbf{size}} \\
%      midrule  
%    \multicolumn{1}{|c|}{} &       &       &       &       &       &       &  \\
%    \multicolumn{1}{|c|}{} &       &       &       &       &       &       &  \\
%    \midrule
%    \textbf{EE} & 0     & 0     & 0     & 0     & 527   & 31.41 & 1456 \\
%    \midrule
%    \textbf{EM1} & 8.55E-02 & 2.55E+02 & 9.70E-01 & 3.93E-03 & 527   & 24.17 & 1288 \\
%    \midrule
%    \textbf{M1M1} & 2.13E+00 & 1.33E+04 & 9.96E-01 & 2.05E-01 & 865   & 14.75 & 1072 \\
%    \midrule
%    \textbf{EM2} & 1.85E-01 & 2.29E+02 & 9.90E-01 & 3.52E-03 & 557   & 22.97 & 1162 \\
%    \midrule
%    \textbf{M2M2} & 1.73E+01 & 1.68E+04 & 1.00E+00 & 2.58E-01 & 600   & 14.4  & 784 \\
%    \midrule
%    \textbf{EM3} & 4.03E-01 & 4.72E+02 & 9.99E-01 & 7.26E-03 & 605   & 24.95 & 1099 \\
%    \midrule
%    \textbf{M3M3} & 1.25E+01 & 1.72E+04 & 1.00E+00 & 2.64E-01 & 598   & 15.31 & 640 \\
%    \midrule
%    \textbf{EM4} & 3.64E-02 & 1.11E+02 & 9.70E-01 & 1.71E-03 & 573   & 21.85 & 1183 \\
%    \midrule
%    \textbf{M4M4} & 6.11E-01 & 6.41E+03 & 9.96E-01 & 9.86E-02 & 313   & 11.17 & 832 \\
%    \midrule
%    \textbf{EM5} & 3.03E-02 & 1.01E+02 & 9.30E-01 & 1.56E-03 & 573   & 22.15 & 1036 \\
%    \midrule
%    \textbf{M5M5} & 6.76E-01 & 8.24E+03 & 9.90E-01 & 1.27E-01 & 250   & 10.69 & 496 \\
%    \midrule
%    \textbf{EX1} & 1.18E-01 & 2.09E+02 & 9.71E-01 & 3.21E-03 & 546   & 31.86 & 1036 \\
%    \midrule
%    \textbf{X1X1} & 2.84E+00 & 1.05E+04 & 9.96E-01 & 1.61E-01 & 558   & 21.33 & 496 \\
%    \midrule
%    \textbf{EX2} & 1.09E-01 & 1.88E+02 & 1.00E+00 & 2.89E-03 & 569   & 23.38 & 994 \\
%    \midrule
%    \textbf{X2X2} & 1.18E+01 & 1.51E+04 & 1.00E+00 & 2.31E-01 & 250   & 13.91 & 400 \\
%    \midrule
%    \textbf{EX3} & 7.96E-02 & 3.48E+02 & 6.15E-01 & 5.35E-03 & 536   & 25.54 & 1036 \\
%    \midrule
%    \textbf{X3X3} & 9.88E-01 & 1.63E+04 & 9.96E-01 & 2.50E-01 & 197   & 15.06 & 496 \\
%    \midrule
%    \textbf{EIn1} & 7.50E-02 & 3.19E+02 & 6.15E-01 & 4.91E-03 & 517   & 26.07 & 994 \\
%    \midrule
%    \textbf{In1In1} & 1.62E+00 & 1.02E+04 & 8.54E-01 & 1.56E-01 & 403   & 14.82 & 400 \\
%    \midrule
%    \textbf{EIn2} & 3.68E-02 & 1.80E+02 & 5.84E-01 & 2.76E-03 & 528   & 28.79 & 1036 \\
%    \midrule
%    \textbf{In2In2} & 4.63E-01 & 8.28E+03 & 8.26E-01 & 1.27E-01 & 340   & 12.56 & 496 \\
%    \midrule
%    \textbf{EIn3} & 1.85E-01 & 2.29E+02 & 9.90E-01 & 3.52E-03 & 556   & 27.96 & 994 \\
%    \midrule
%    \textbf{In3In3} & 1.73E+01 & 1.68E+04 & 1.00E+00 & 2.58E-01 & 404   & 23.92 & 400 \\
%    \bottomrule
%    \end{tabular}   %   }
%\label{table:8X8Array}
%\end{table}%


 For our approximate designs, a specific approximation degree, from 1 to \textit{2n}, rather than \textit{n}, may be chosen based on the maximum error allowed for a specific application, where in\cite{SALSA} \cite{SASIMI}, it is mentioned that it is suitable to chose a value of 10\% for Maximum ED and 0.5\% for MED. Figure \ref{fig:error_8x8Array} shows the ER, NMED and MRED for various 8x8 array multipliers. It is clear that fully approximate multipliers have high NMED. \textit{EM5} has the lowest NMED, and \textit{EM4} has a close-to-minimal NMED. Designs with high NMED have a high MRED too. It can be observed that \textit{EIn2} exhibits the lowest ER. Also, \textit{EX3} and \textit{EIn1} have the same close-to-minimal ER. 

 \begin{figure}[!h]
 \centering
\includegraphics[width=1.0\textwidth , height=5cm]{8AERROR.png}
\caption{ER x$10^{-2}$, NMED x$10^{-3}$ and MRED x$10^{-1}$ of 8x8 Array Multiplier}
\label{fig:error_8x8Array}
\end{figure} 

 \begin{figure}[!h]
 \centering
\includegraphics[width=1.0\textwidth, height=5cm]{8A-P.png}
\caption{Area and PDP Reduction of 8x8 Array Multiplier}
\label{fig:PDP_Area_NMED_8x8Array}
\end{figure}


 As shown in Table \ref{table:8X8Array} and Figure \ref{fig:error_8x8Array}, there is no single design that is superior in all design metrics. Therefore, a Pareto-analysis for the improvements in area and PDP is shown for the different  designs proposed throughout this work. \textit{X3X3} has the lowest delay, and \textit{M5M5} and \textit{X2X2} also exhibit a low delay. \textit{M5M5}, \textit{M4M4} and \textit{In2In2} exhibit the lowest power consumption among the 22 different designs. The size of the approximate multiplier exhibits a linear relationship with the degree of approximation. Thus, \textit{X2X2}, \textit{In1In1} and \textit{In3In3}, have the smallest size.
   
%As shown in Table \ref{table:8X8Array}, there is no single design that is superior in all design metrics. Therefore, improvements in design metrics including area and power-delay-product are shown for different proposed designs (8x8, 16x16, tree and array multiplier) throughout this work.



Figure \ref{fig:PDP_Area_NMED_8x8Array} shows the area and PDP reduction of 8x8 array multipliers. The best designs are located on the bottom left corner. \textit{M5M5} is a Pareto-design with PDP reduction of 84\% and area reduction of 65\%. The design \textit{X3X3} is Non-Pareto because it has the same area reduction as the \textit{M5M5} but with a smaller PDP reduction. However, we have to consider other \textit{error metrics}. Some designs such as \textit{EX1} have increased PDP due to excessive switching activity compared to the original design.
 

 %
 


  %Approximate multipliers, including \textit{X2X2}, \textit{In1In1} and \textit{In3In3}, which are based on FA with 6 transistors, exhibit 73\% area reduction with PDPs of 79\%, 64\% and 10\%, respectively. Clearly fully designs have high area and PDP reduction. Some designs such as \textit{EX1} have increased PDP due to excessive switching activity compared to original design.

%As depicted in Figure \ref{fig:PDP_Area_NMED_8x8Array}, \textit{M5M5} has the highest PDP reduction (83.8\%) with 65\% area reduction. The area and PDP reduction of \textit{X3X3} are almost identical to \textit{M5M5} but \textit{X3X3} is better in terms of NMED. Approximate multipliers, including \textit{X2X2}, \textit{In1In1} and \textit{In3In3}, which are based on FA with 6 transistors, exhibit 72.5\% area reduction with PDPs of 78.9\%, 63.9\% and 9.6\%, respectively. It can be noticed that most of the fully approximate 8x8 array multipliers have high PDP reduction and area reduction with relatively high NMED. Similarly, approximate 8x8 array multipliers, with approximation in LSBs only, have low PDP reduction and area reduction with relatively low NMED. Clearly, the best designs in terms of PDP reduction are \textit{M5M5}, \textit{X3X3} and \textit{X2X2} since they are fully approximate with low power consumption. The best designs in terms of area reduction are \textit{In3In3}, \textit{In1In1} and \textit{X2X2} since they are fully approximate based on 6 transistor cells. Also, the best designs based on the NMED are \textit{EM5}, \textit{EM4} and \textit{EIn2}, with low degree of approximation.

%\includegraphics[width=9cm]{image010.png}


\subsection{\textbf{8x8 Tree Multiplier}} \label{sec:Tree8}

The Wallace multiplier\cite{Parhami} is an efficient parallel multiplier that is composed of a tree of half adders (HAs) and FAs. The main idea is that, the adders in each layer operate in parallel without carry propagation until the generation of two rows of partial products. The design space for approximate 8x8 tree multipliers \cite{Parhami} is also quite large, depending on the \textit{compressor type} and \textit{approximation degree}. To avoid the exponentially growing design space, we choose to use compressors of the same type in the multiplier design. Also, we use two options for approximation degree: i) all compressors are approximate, and ii) compressors that contribute to the lowest significant 50\% of the resultant bits are approximated to maintain an acceptable accuracy. Thus, based on the four shortlisted compressors, explained in Section \ref{sec:ApproxFA}, we compared 8 options for approximate 8x8 tree multipliers and the results are given in Table \ref{table:8X8Tree}. The name of the multiplier consists of three parts. For example, CEM1 represents a compressor based multiplier (C), where the most significant part is based on an exact (E) compressor and the least significant part is composed of the mirror adder 1 (M1) based compressor. As shown in Table \ref{table:8X8Tree}, there is no single design superior is all metrics, but some designs are the best wrt some few metrics. 

Figure \ref{fig:error_8x8Tree} shows the ER, NMED and MRED for various 8x8 tree multipliers. Fully approximate designs have higher NMED and MRED than partially approximate designs. The designs based on \textit{InX1} (\textit{CEIn1} and \textit{CIn1In1}) exhibit the lowest ER. \textit{CM3M3} have the highest MRED. The designs based on \textit{AMA5} have the lowest delay and power consumption due to their simple structures. 

As depicted in Figure \ref{fig:PDP_Area_NMED_8x8Tree} which shows area and PDP reduction, the best designs are on the left bottom corner, i.e., \textit{CM5M5} is a Pareto-design with maximum area and maximum PDP reduction. However, \textit{CEM5} is a non Pareto-design because it has less reduction. Few designs on the right side of the figure have a PDP value greater than the exact design, which makes them unsuitable for low-power design usage.

% \textit{CEIn1} multiplier has the smallest ER with relatively small NMED, and this goes with InXA1 FA characteristics. \textit{CEM5} has the smallest NMED. The multiplier with the lowest delay, and the lowest power dissipation is \textit{CM5M5}, \textcolor{red}{due to its simple internal structure}. Also, \textit{CEM5} has a relatively low delay. \textit{CX2X2} and \textit{CIn1In1} have the lowest number of transistors since they are based on small approximate cells.


%\begin{table}[!t]
%\centering
% \caption{8x8 Approximate Tree Multiplier}
% %\resizebox{\columnwidth}{!}{%
%  \scalebox{0.85}{
%   \begin{tabular}{|c|c|c|c|c|c|} \hline
%\textbf{Type} & \textbf{ER} &\textbf{NMED} &\textbf{Delay}(PS) &	\textbf{POWER}($\mu$W)&	\textbf{SIZE}  \\   \hline \hline
%
%\textbf{CEE}	&0.00	&0.00	  & 508	&21.98	&1218 \\   \hline
%\textbf{CEM3}&	1.00&	9.30x10\textsuperscript{-3}&	537	&19.65	&912  \\   \hline
%\textbf{CM3M3}&	1.000&	2.16x10\textsuperscript{-1}&	560	&\cellcolor{yellow}\textbf{16.27}	&606  \\   \hline
%\textbf{CEM5}&	9.79x10\textsuperscript{-1}&	\cellcolor{yellow}\textbf{2.40x10\textsuperscript{-3}}&\cellcolor{yellow}\textbf{356}	&18.63	&858  \\   \hline
%\textbf{CM5M5}&	9.99x10\textsuperscript{-1}&	8.18x10\textsuperscript{-2}&	\cellcolor{yellow}\textbf{282}	&\cellcolor{yellow}\textbf{13.99}	&498  \\   \hline
%\textbf{CEX2}&	9.97x10\textsuperscript{-1}&	5.70x10\textsuperscript{-3}&	525	&23.52	&822  \\   \hline
%\textbf{CX2X2}&	1.00&	1.38x10\textsuperscript{-1}&	513	&22.6	&\cellcolor{yellow}\textbf{426}  \\   \hline
%\textbf{CEIn1}&	\cellcolor{yellow}\textbf{8.73x10\textsuperscript{-1}}&	\cellcolor{yellow}\textbf{4.80x10\textsuperscript{-3}}&	505	&25.12	&822  \\   \hline
%\textbf{CIn1In1}&\cellcolor{yellow}\textbf{9.75x10\textsuperscript{-1}}&	7.81x10\textsuperscript{-2}&	500	&26.89	&\cellcolor{yellow}\textbf{426}  \\   \hline
%\end{tabular}  }
%\label{table:8X8Tree}
%\end{table}


\begin{table}[!t]
\centering
 \caption{8x8 Approximate Tree Multiplier}
 %\resizebox{\columnwidth}{!}{%
  \scalebox{0.7}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \toprule
   % \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{4.055em}|}{\textbf{Delay (ps)}} & \multicolumn{1}{p{4.055em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{4.055em}|}{\textbf{size}} \\
             \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{2.555em}|}{\textbf{Delay (ps)}} & \multicolumn{1}{p{2.78em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{2.11em}|}{\textbf{size}} \\
             
    \midrule
    \textbf{CEE} & 00 & 00 & 00 & 00 & 508   & 21.98 & 1218 \\
    \midrule
    \textbf{CEM3} & 4.76E-01 & 6.05E+02 & 1.00E+00 & 9.30E-03 & 537   & 19.65 & 912 \\
    \midrule
    \textbf{CM3M3} & 1.06E+01 & 1.41E+04 & 1.00E+00 & 2.16E-01 & 560   & 16.27 & 606 \\
    \midrule
    \textbf{CEM5} & 4.76E-02 & 1.54E+02 & 9.79E-01 & 2.40E-03 & 356   & 18.63 & 858 \\
    \midrule
    \textbf{CM5M5} & 5.16E-01 & 5.32E+03 & 9.99E-01 & 8.18E-02 & 282   & 13.99 & 498 \\
    \midrule
    \textbf{CEX2} & 3.28E-01 & 3.68E+02 & 9.97E-01 & 5.70E-03 & 525   & 23.52 & 822 \\
    \midrule
    \textbf{CX2X2} & 7.35E+00 & 8.95E+03 & 1.00E+00 & 1.38E-01 & 513   & 22.6  & 426 \\
    \midrule
    \textbf{CEIn1} & 9.03E-02 & 3.10E+02 & 8.73E-01 & 4.80E-03 & 505   & 25.12 & 822 \\
    \midrule
    \textbf{CIn1In1} & 5.08E-01 & 5.08E+03 & 9.75E-01 & 7.81E-02 & 500   & 26.89 & 426 \\
    \bottomrule
\hline
\end{tabular}  }
\label{table:8X8Tree}
\end{table}

%As depicted in Figure \ref{fig:PDP_Area_NMED_8x8Tree}, best designs are on left bottom corner. i.e., \textit{CM5M5} and \textit{CX2X2} are Pareto-design while \textit{CEM5} in non Pareto-design. % and \textit{CM3M3}, and the best designs in terms of area reduction are on the bottom including are \textit{CIn1In1}, \textit{CX2X2} and \textit{CM5M5}. some designs have increased PDP value compared to exact design, this is due to excess switching activity that could be reduced for another set of input data.





%\subsection{\textbf{Discussion}}
%To evaluate the characteristics of the proposed multipliers, simulation is performed using Cadence's Spectre in TSMC65nm (CRN65LP) process with a standard supply voltage (V\textsubscript{dd}) of 1.0V at room temperature. Circuit inputs are provided by independent voltage sources, and a load of 10fF is utilized. It can be observed from our results that the 8x8 exact tree multiplier exhibits lower delay, power and size compared to the exact 8x8 array multiplier. Delay is reduced from O(n) to O(log\textsubscript{2}n) due to the circuit structure. Also, uneven signal transitions for the FAs cause glitches that increases the power consumption of array multipliers. Compressors are used to avoid such problems in the tree multiplier. The 8x8 array and tree multiplier designs, based on AMA5, have the lowest delay and power consumption, due to the basic structure of the FA cell, which is composed of two buffers only. Also, they have the lowest NMED and a small size (based on a FA with 8 transistors). Regarding accuracy, the designs based on \textit{InXA1} have the lowest ER and NMED. Similarly, the designs based on the 6 transistors FA (\textit{AXA2}, \textit{InXA1} and \textit{InXA3}), have the minimal size. Thus, it can be observed that the characteristics of approximate FA are generally depicted in the corresponding approximate multipliers as well. 


%\textit{CEM5} and \textit{CEIn1} provide the best NMED.
%\includegraphics[width=9cm]{image058.png}


\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{8TT.png}
\includegraphics[width=1.0\textwidth, height=5cm]{8Terror.png}
\caption{ER x$10^{-2}$, NMED x$10^{-3}$ and MRED x$10^{-1}$ of 8x8 Tree Multiplier}
\label{fig:error_8x8Tree}
\end{figure}


\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{8TT.png}
\includegraphics[width=1.0\textwidth, height=5cm]{8C-P.png}
\caption{Area and PDP Reduction of 8x8 Tree Multiplier}
\label{fig:PDP_Area_NMED_8x8Tree}
\end{figure}


==> Arxiv-Online-Comparative-TR uploaded/Conclusion.tex <==
\section{\textbf{Conclusions}} \label{sec:conclusion}

In this report, we designed, evaluated and compared different approximate multipliers, based on approximation in partial product summation. The design space of approximate multipliers is found to be primarily dependent on the type of the approximate FA used, the architecture, and the placement of 8x8 sub-modules in the higher-order \textit{n}x\textit{n} multipliers. The proposed designs are compared based on PDP, area, delay, power, quality( ER, NMED and MRED). Various optimal designs have been identified in terms of the considered  design metrics. An image blending application is used to compare the proposed multiplier designs in terms of SNR and PDP. Our designs show comparative results compared to 24 different approximate designs reported in \cite{Jiang}. In the future, we plan to investigate the design space of higher-order multiplier modules (e.g., 64x64) using the already considered metrics and configurations. Moreover, we also plan to evaluate the possibility of having mixed FAs in the 8x8 multiplier block.




==> Arxiv-Online-Comparative-TR uploaded/HigherOrderBlock.tex <==

\section{\textbf{ Higher-Order Multiplier Configuration}}   \label{sec:MainModule}

The 8x8 multiplier basic modules can be used to construct higher-order target multiplier modules. In this report, we use the example of designing a 16x16 multiplier to illustrate this process. The partial product tree of the 16x16 multiplication can be broken down into four products of 8x8 modules, which can be executed concurrently, as shown in Figure \ref{fig:recursive}.

\begin{figure}[h!]
\centering
\includegraphics[width=6cm, height=3cm]{cc1.png}
\caption{16x16 Multiplier}
\label{fig:recursive}
\end{figure}

In the case of high requirements of accuracy, an exact 8x8  multiplier can be used for the three most significant products, i.e., AHxBH, AHxBL, and ALxBH, and any one of the approximate designs can be used for the least significant product, i.e., ALxBL. For low accuracy requirements, only one 8x8 exact multiplier can be used for the most significant product, i.e., AHxBH, and any of the other approximate designs can be used for the three least significant products, i.e., AHxBL, ALxBH, and ALxBL. Modules that contribute to the lowest significant 50\% of the resultant bits are approximated to maintain accuracy as recommended by \cite{Vaibhav} \cite{Reddy} \cite{Shao}\cite{FEMTO}.

We choose to design 16x16 multipliers with an exact AHxBH multiplier, and with exact MSBs and approximate LSBs for AHxBL and ALxBH, and a fully approximate or approximate in LSBs only ALxBL. Any other approximation degree can be found based on the required quality function (maximum error, area, power or delay).
Therefore, when the 16x16 multipliers are explained, the types of AHxBH, AHxBL and ALxBH are eliminated  from the name, and only the type of ALxBL is used in the name of the multiplier.

%The following 16X16 multipliers have been constructed based on four 8X8 multipliers where each 16X16 type is (X-Y-Z) where X represent type of 8X8 AHxBH, Y represent the type of 8X8 AHxBL and ALxBH, and Z represent the type of 8X8 ALxBL.

\subsection{\textbf{16x16 Array Multiplier}} \label{sec:Array16}

Table \ref{table:16X16Array} shows the simulation results for 16x16 approximate array multipliers, which shows similarities with Table \ref{table:8X8Array}. The multiplier name is based on the type of ALxBL module. Figures \ref{fig:ER_16x16Array}, \ref{fig:NMED_16x16Array} and \ref{fig:MRED_16x16Array} show the ER, NMED and MRED for 16x16 array multipliers, respectively. It can be observed that \textit{16M1M1} is the most accurate design with the lowest ER and lowest NMED. \textit{16EIn2} is the second accurate design with low ER and NMED. For NMED, the best designs are \textit{16M1M1}, \textit{16EIn2} and \textit{16In2In2}. Designs with high NMED show a high MRED value. \textit{EIn1In1} and \textit{16In3In3} have the lowest delay. Fully approximate designs exhibit the minimal delay. Generally, designs based on approximate mirror adders have the lowest power consumption, due to the elimination of static power dissipation. Since, the design size grows linearly with the FA size, fully approximate designs based on 6 transistors  cells including \textit{16X2X2}, \textit{16In1In1} and \textit{16In3In3} have the smallest number of transistors. Also, fully approximate designs including \textit{16M5M5}, \textit{16X1X1}, \textit{16X3X3} and \textit{16In2In2}, based on 8 transistors FAs, have a very small size as well.  Finally, the best designs regarding area reduction are \textit{16In1In1}, \textit{16X2X2} and \textit{16In3In3}. 

%Regarding power consumption, \textit{16M4M4} and \textit{16M5M5} have similar minimal power consumption with 105.1$\mu$W. \textit{InM2M2}, \textit{InEM4} and \textit{16EM5} have close power consumption, which is 116.5$\mu$W, 118.4$\mu$W and 118.8$\mu$W, respectively. 

%\begin{table}[t!]
%\centering
% \caption{16x16 Approximate Array Multiplier }
%%\resizebox { \columnwidth}{!} {
%  %\resizebox{\linewidth}{!}
%  
%   \scalebox{0.85}{
%   \begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\textbf{Type} & \textbf{ER} &\textbf{NMED} &\textbf{Delay}(PS) &	\textbf{POWER}($\mu$W)&	\textbf{SIZE}  \\   \hline \hline
%
%\textbf{16EE}&	0&	0.00&	514&	156.8&	5824 \\   \hline
%\textbf{16EM1}&	9.4x10\textsuperscript{-1}&	7.69x10\textsuperscript{-10}&	534&	130.1&	5320 \\   \hline 
%\textbf{16M1M1}&\cellcolor{yellow}\textbf{1.76x10\textsuperscript{-2}}&	\cellcolor{yellow}\textbf{1.10x10\textsuperscript{-11}}&	526	&\textbf{118.4}&	5104 \\   \hline 
%\textbf{16EM2}&	1&	1.82x10\textsuperscript{-5}&533&128.4 &	4942 \\   \hline 
%\textbf{16M2M2} &	1&	2.28x10\textsuperscript{-5}&\cellcolor{yellow}\textbf{477}&	\cellcolor{yellow}\textbf{116.5}&	4562 \\   \hline 
%\textbf{16EM3}	&1	&6.16x10\textsuperscript{-5}&519	&131.6	&4753 \\   \hline 
%\textbf{16M3M3}	&1	&6.45x10\textsuperscript{-5}&\textbf{490}&\textbf{120.4}&4294 \\   \hline 
%\textbf{16EM4}	&9.285x10\textsuperscript{-1}&	5.04x10\textsuperscript{-10}&	522&\textbf{118.8} &	5005 \\   \hline 
%\textbf{16M4M4}	&9.793x10\textsuperscript{-1}&5.11x10\textsuperscript{-10}&	\textbf{506}	&\cellcolor{yellow}\textbf{105.1}	&4654 \\   \hline 
%\textbf{16EM5}	&9.335x10\textsuperscript{-1}&5.30x10\textsuperscript{-10}&533	&\textbf{119}&	4564 \\   \hline 
%\textbf{16M5M5}	&9.335x10\textsuperscript{-1}&5.30x10\textsuperscript{-10}&535&	\cellcolor {yellow}\textbf{105.1}&	4022 \\   \hline \hline
%\textbf{16EX1}	&9.509x10\textsuperscript{-1}&7.43x10\textsuperscript{-10}&513	&154.9&	4564 \\   \hline 
%\textbf{16X1X1}	&9.793x10\textsuperscript{-1}&8.34x10\textsuperscript{-10}&520	&138.5	&4024 \\   \hline 
%\textbf{16EX2}	&1&	6.07x10\textsuperscript{-6}&521&138	&4438 \\   \hline 
%\textbf{16X2X2}	&1&	9.11x10\textsuperscript{-6}&514	&127.4&\cellcolor{yellow}\textbf{3844} \\   \hline
%\textbf{16EX3}	&9.646x10\textsuperscript{-1}&1.09x10\textsuperscript{-9}	&515	&134	&4564 \\   \hline 
%\textbf{16X3X3}	&9.793x10\textsuperscript{-1}&1.27x10\textsuperscript{-9}&	518&	121.8&	4024 \\   \hline \hline
%\textbf{16EIn1}	&\textbf{5.239x10\textsuperscript{-1}}&5.04x10\textsuperscript{-10}	&519	&134.2&	4438 \\   \hline 
%\textbf{16In1In1}&	\textbf{6.09x10\textsuperscript{-1}}	&5.43x10\textsuperscript{-10}&	\cellcolor{yellow}\textbf{408}&121.7&	\cellcolor{yellow}\textbf{3844} \\   \hline 
%\textbf{16EIn2}	&\cellcolor{yellow}\textbf{2.137x10\textsuperscript{-1}}&\cellcolor{yellow}	\textbf{1.03x10\textsuperscript{-10}}	&537	&146.9	&4564 \\   \hline 
%\textbf{16In2In2}&	\cellcolor{yellow}\textbf{4.29x10\textsuperscript{-1}}	&\cellcolor{yellow}\textbf{1.42x10\textsuperscript{-10}}&\textbf{500}&	126.4&	4024 \\   \hline
%\textbf{16EIn3}	&1	&1.82x10\textsuperscript{-5}	&527	&157.6	&4438 \\   \hline 
%\textbf{16In3In13}	&1&	2.28x10\textsuperscript{-5}&	\cellcolor{yellow}\textbf{412}&	153.2&	\cellcolor{yellow}\textbf{3844} \\   \hline 
%\end{tabular} 
% }
%\label{table:16X16Array}
%\end{table}

\begin{table}[t!]
 \centering
 \caption{16x16 Approximate Array Multiplier}
%\resizebox { \columnwidth}{!} {
  %\resizebox{\linewidth}{!}
   \scalebox{0.7}{ 
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \toprule
   % \multicolumn{1}{|c|}{\multirow{2}[2]{*}{\textbf{Type}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{MRED}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{MED}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{ER}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{NMED}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{Delay (ps)}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{POWER ($\mu$W)}}} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{\textbf{size}}} \\
       \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{2.555em}|}{\textbf{Delay (ps)}} & \multicolumn{1}{p{2.78em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{2.11em}|}{\textbf{size}} \\
       %   &       &       &       &       &       &       &  \\
    \midrule
    \textbf{16EE} & 00 & 00 & 00 & 00 & 514   & 156.8 & 5824 \\
    \midrule
    \textbf{16EM1} & 1.19E-02 & 6.31E+04 & 9.44E-01 & 7.69E-10 & 534   & 130.1 & 5320 \\
    \midrule
    \textbf{16M1M1} & 1.71E-04 & 1.33E+03 & 1.76E-02 & 1.10E-11 & 526   & 118.4 & 5104 \\
    \midrule
    \textbf{16EM2} & 2.82E+02 & 1.14E+05 & 1.00E+00 & 1.82E-05 & 533   & 128.4 & 4942 \\
    \midrule
    \textbf{16M2M2} & 3.53E+02 & 1.33E+05 & 1.00E+00 & 2.28E-05 & 477   & 116.5 & 4562 \\
    \midrule
    \textbf{16EM3} & 9.53E+02 & 3.34E+05 & 1.00E+00 & 6.16E-05 & 519   & 131.6 & 4753 \\
    \midrule
    \textbf{16M3M3} & 9.98E+02 & 3.51E+05 & 1.00E+00 & 6.45E-05 & 490   & 120.4 & 4294 \\
    \midrule
    \textbf{16EM4} & 7.80E-03 & 3.36E+04 & 9.29E-01 & 5.04E-10 & 522   & 118.8 & 5005 \\
    \midrule
    \textbf{16M4M4} & 7.90E-03 & 3.32E+04 & 9.79E-01 & 5.11E-10 & 506   & 105.1 & 4654 \\
    \midrule
    \textbf{16EM5} & 8.20E-03 & 4.06E+04 & 9.34E-01 & 5.30E-10 & 533   & 119   & 4564 \\
    \midrule
    \textbf{16M5M5} & 8.20E-03 & 4.06E+04 & 9.34E-01 & 5.30E-10 & 535   & 105.1 & 4024 \\
    \midrule
    \textbf{16EX1} & 1.15E-02 & 5.22E+04 & 9.51E-01 & 7.43E-10 & 513   & 154.9 & 4564 \\
    \midrule
    \textbf{16X1X1} & 1.29E-02 & 5.74E+04 & 9.79E-01 & 8.34E-10 & 520   & 138.5 & 4024 \\
    \midrule
    \textbf{16EX2} & 9.40E+01 & 5.96E+04 & 1.00E+00 & 6.07E-06 & 521   & 138   & 4438 \\
    \midrule
    \textbf{16X2X2} & 1.41E+02 & 6.85E+04 & 1.00E+00 & 9.11E-06 & 514   & 127.4 & 3844 \\
    \midrule
    \textbf{16EX3} & 1.69E-02 & 9.09E+04 & 9.65E-01 & 1.09E-09 & 515   & 134   & 4564 \\
    \midrule
    \textbf{16X3X3} & 1.97E-02 & 1.05E+05 & 9.79E-01 & 1.27E-09 & 518   & 121.8 & 4024 \\
    \midrule
    \textbf{16EIn1} & 7.80E-03 & 4.57E+04 & 5.24E-01 & 5.04E-10 & 519   & 134.2 & 4438 \\
    \midrule
    \textbf{16In1In1} & 8.40E-03 & 4.93E+04 & 6.09E-01 & 5.43E-10 & 408   & 121.7 & 3844 \\
    \midrule
    \textbf{16EIn2} & 1.60E-03 & 8.08E+03 & 2.14E-01 & 1.03E-10 & 537   & 146.9 & 4564 \\
    \midrule
    \textbf{16In2In2} & 2.20E-03 & 1.13E+04 & 4.29E-01 & 1.42E-10 & 500   & 126.4 & 4024 \\
    \midrule
    \textbf{16EIn3} & 2.82E+02 & 1.14E+05 & 1.00E+00 & 1.82E-05 & 527   & 157.6 & 4438 \\
    \midrule
    \textbf{16In3In13} & 3.53E+02 & 1.33E+05 & 1.00E+00 & 2.28E-05 & 412   & 153.2 & 3844 \\
    \bottomrule

 \end{tabular} 
  }
\label{table:16X16Array}
\end{table}



%\textit{16In1In1} design has the highest PDP reduction (38.39\%) and highest area reduction (34\%). \textit{16M4M4} has a high PDP (34.02\%), and moderate area reduction (20.1\%). Both designs have a high accuracy with low NMED (almost 5x10\textsuperscript{-10}). \textit{16In1In1}, \textit{16In3In3} and \textit{16X2X2}, have the highest area reduction with PDP reduction of 38.39\%, 21.68\% and 18.75\%, respectively.


 %Fully approximate designs exhibit the minimal delay due to reduced circuit complexity. Generally, designs based on approximate mirror adders have the lowest power consumption, due to the elimination of static power dissipation. Since, the design size grows linearly with the FA size, fully approximate designs based on 6 transistors cells have the smallest area. 





\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16A_ER.png}
\caption{ER x$10^{-2}$ of 16x16 Array Multiplier}
\label{fig:ER_16x16Array}
\end{figure}


\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16A_NMED.png}
\caption{NMED x$10^{-5}$ of 16x16 Array Multiplier}
\label{fig:NMED_16x16Array}
\end{figure}

\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16A_MRED.png}
\caption{MRED x$10^{-1}$of 16x16 Array Multiplier}
\label{fig:MRED_16x16Array}
\end{figure}



\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16A-P.png}
\caption{Area and PDP Reduction of 16x16 Array Multiplier}
\label{fig:PDP_Area_NMED_16x16Array}
\end{figure}

As depicted in Figure \ref{fig:PDP_Area_NMED_16x16Array} which shows the reduction in area and PDP for 16x16 array multipliers, the best designs are on the lower left corner, i.e., \textit{16In1In1} and \textit{16In3In3} are Pareto-designs while \textit{16M4M4} is a non-Pareto design. Designs with negative PDP reduction values, indicate a power or delay larger than the exact design.


%Similar to approximate 8X8 array multipliers, Figure \ref{fig:PDP_Area_NMED_16x16Array} show a high PDP and area reduction with high NMED generally for 16X16 approximate array multipliers, which have a high degree of approximation




% \textit{16CEIn1} has the lowest ER with a relatively low NMED. \textit{16CEM5} has the lowest NMED with low ER. Regarding delay, \textit{16CEIn1} and \textit{16CIn1In1} exhibit the lowest delay. \textit{16CM5M5} has the lowest power consumption, and \textit{16CM3M3} has close-to-minimal power consumption. The designs with minimal number of transistors are \textit{16CX2X2} and \textit{16CIn1In1}.


%\begin{table}[t!]
% \centering
% \caption{16x16 Approximate Tree Multiplier}
%%\resizebox { \columnwidth}{!} {
%  %\resizebox{\linewidth}{!}
%   \scalebox{0.85}{ 
%   \begin{tabular}{|c|c|c|c|c|c|}
%\hline
%
%\textbf{Type} & \textbf{ER} &\textbf{NMED} &\textbf{Delay}(PS) &	\textbf{POWER}($\mu$W)&	\textbf{SIZE}  \\   \hline \hline\
%\textbf{16CEE}	&0.0&	0.0& 	680&	100.8&	4872 \\   \hline 
%\textbf{16CEM3}	&1.00	&3.00x10\textsuperscript{-3}	&663	&93.57	&3954 \\   \hline 
%\textbf{16CM3M3}	&1.00	&3.10x10\textsuperscript{-3}&693	&\cellcolor{yellow}\textbf{90.6}	&\textbf{3648} \\   \hline 
%\textbf{16CEM5}	&\textbf{9.41x10\textsuperscript{-1}}	&\cellcolor{yellow}\textbf{2.52x10\textsuperscript{-8}}	&\textbf{585}	&\textbf{92.48} &	3792 \\   \hline 
%\textbf{16CM5M5}	&9.79x10\textsuperscript{-1}	&\textbf{2.56x10\textsuperscript{-8}}	&670	&\cellcolor{yellow}\textbf{86.98}	&\textbf{3432} \\   \hline 
%\textbf{16CEX2}	&1.00	&2.30x10\textsuperscript{-3}&685	&115	&3684 \\   \hline 
%\textbf{16CX2X2}	&1.00	&2.40x10\textsuperscript{-3}	&671	&114.3	&\cellcolor{yellow}\textbf{3288}  \\   \hline 
%\textbf{16CEIn1}	&\cellcolor{yellow}\textbf{8.22x10\textsuperscript{-1}}&	\cellcolor{yellow}\textbf{4.83x10\textsuperscript{-8}}&	\cellcolor{yellow}\textbf{516}&	112.5&	3684 \\   \hline 
%\textbf{16CIn1In1}	&\cellcolor{yellow}\textbf{9.04x10\textsuperscript{-1}}&	4.98x10\textsuperscript{-8}&	\cellcolor{yellow}\textbf{527}&	114.3&	\cellcolor{yellow}\textbf{3288} \\   \hline 
% \end{tabular} 
%  }
%\label{table:16X16Tree}
%\end{table}



\subsection{\textbf{16x16 Tree Multiplier}}  \label{sec:Tree16}

Table \ref{table:16X16Tree} depicts the characterization for 16x16 approximate tree multipliers, which to some degree shows similarities to Table \ref{table:8X8Tree}. The design \textit{16CM5M5} has the lowest power consumption. Figures \ref{fig:ER_16x16Tree}, \ref{fig:NMED_16x16Tree} and  \ref{fig:MRED_16x16Tree} shows the ER, NMED and MRED for 16x16 tree multipliers, respectively. \textit{16CEIn1} and \textit{16CIn1In1} have the lowest ER, delay and area. The same designs have high NMED and MRED. As depicted in Figure \ref{fig:PDP_Area_NMED_16x16Tree} which shows area and PDP reduction, the designs on the lower left corner are superior, i.e., \textit{16CEM5}, \textit{16CEIn1} and \textit{16CM5M5} are all Pareto-designs while \textit{16CEM3} is a non-Pareto design.


\begin{table}[t!]
 \centering
 \caption{16x16 Approximate Tree Multiplier}
%\resizebox { \columnwidth}{!} {
  %\resizebox{\linewidth}{!}
   \scalebox{0.7}{ 
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
    \toprule
    \textbf{Type} & \multicolumn{1}{p{4.055em}|}{\textbf{MRED}} & \multicolumn{1}{p{4.055em}|}{\textbf{MED}} & \multicolumn{1}{p{4.055em}|}{\textbf{ER}} & \multicolumn{1}{p{4.055em}|}{\textbf{NMED}} & \multicolumn{1}{p{2.555em}|}{\textbf{Delay (ps)}} & \multicolumn{1}{p{2.78em}|}{\textbf{Power ($\mu$W)}} & \multicolumn{1}{p{2.11em}|}{\textbf{size}} \\
    \midrule
    \textbf{16CEE} & 00 & 00 & 00 & 00 & 680   & 100.8 & 4872 \\
    \midrule
    \textbf{16CEM3} & 1.07E+03 & 4.64E+04 & 1.00E+00 & 3.00E-03 & 663   & 93.57 & 3954 \\
    \midrule
    \textbf{16CM3M3} & 1.11E+03 & 4.80E+04 & 1.00E+00 & 3.10E-03 & 693   & 90.6  & 3648 \\
    \midrule
    \textbf{16CEM5} & 9.10E-03 & 3.90E-01 & 9.41E-01 & 2.52E-08 & 585   & 92.48 & 3792 \\
    \midrule
    \textbf{16CM5M5} & 9.30E-03 & 3.96E-01 & 9.79E-01 & 2.56E-08 & 670   & 86.98 & 3432 \\
    \midrule
    \textbf{16CEX2} & 8.37E+02 & 3.56E+04 & 1.00E+00 & 2.30E-03 & 685   & 115   & 3684 \\
    \midrule
    \textbf{16CX2X2} & 8.65E+02 & 3.71E+04 & 1.00E+00 & 2.40E-03 & 671   & 114.3 & 3288 \\
    \midrule
    \textbf{16CEIn1} & 1.74E-02 & 7.47E-01 & 8.22E-01 & 4.83E-08 & 516   & 112.5 & 3684 \\
    \midrule
    \textbf{16CIn1In1} & 1.79E-02 & 7.70E-01 & 9.04E-01 & 4.98E-08 & 527   & 114.3 & 3288 \\
    \bottomrule

 \end{tabular} 
  }
\label{table:16X16Tree}
\end{table}
 
 
 
 \begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16T_ER.png}
\caption{ER x$10^{-2}$ of 16x16 Tree Multiplier}
\label{fig:ER_16x16Tree}
\end{figure}


\begin{figure}[h!]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16T_NMED.png}
\caption{NMED x$10^{-3}$ of 16x16 Tree Multiplier}
\label{fig:NMED_16x16Tree}
\end{figure}

\begin{figure}[!h]
\centering
%\includegraphics[width=9cm]{16A.png}
\includegraphics[width=1.0\textwidth, height=5cm]{16T_MRED.png}
\caption{MRED x$10^{-1}$of 16x16 Tree Multiplier}
\label{fig:MRED_16x16Tree}
\end{figure}


 %\includegraphics[width=9cm]{image023.png} 
\begin{figure}[!h]
\centering
\includegraphics[width=1.0\textwidth, height=5cm]{16C-P.png}
%\includegraphics[width=9cm]{166.png}
\caption{Area and PDP Reduction of 16x16 Tree Multiplier}
\label{fig:PDP_Area_NMED_16x16Tree}
\end{figure}




%As depicted in Figure \ref{fig:PDP_Area_NMED_16x16Tree}, designs \textit{16CEM5} has the highest PDP reduction, high area reduction and the lowest NMED. \textit{16CX2X2} and \textit{16CIn1In1} have the highest area reduction. Designs based on AXA2 FA have high power consumption, thus their PDP is higher than exact design. The best designs regarding PDP reduction are \textit{16CEM5}, \textit{16CEIn1} and \textit{16CM5M5}. The best designs with respect to the area reduction are \textit{16CIn1In1} and\textit{16X2X2}. For NMED, the best designs are \textit{16CEM5}, \textit{16CM5M5} and \textit{16CEIn1}.



\subsection{\textbf{Discussion and Comparison}}  \label{sec:Dis}
%Higher-order multiplier modules, have different characteristics, for various design configuration options, such as: i) The type of FA used:Designs based on 
The considered approximate multipliers are implemented using Cadence's Spectre based on TSMC65nm process, with V\textsubscript{dd} = 1.0V at T=27C\textsuperscript{o}. The circuit inputs are provided by independent voltage sources, and a load of 10fF is utilized. We evaluated and compared the design characteristics (Area, Power and Delay). As shown in Tables \ref{table:8X8Array} and \ref{table:8X8Tree}, the 8x8 exact tree multiplier exhibits lower delay, power and size compared to the exact 8x8 array multiplier. 

%Delay is reduced from O(n) to O(log\textsubscript{2}n) due to the circuit structure.

%Also, uneven signal transitions for the FAs cause glitches that increases the power consumption of array multipliers. Compressors are used to avoid such problems in the tree multiplier.

Several multiplier designs, based on \textit{AMA5}, have the lowest delay and power consumption, due to the basic structure of the FA cell, which is composed of two buffers only. Also, they have the lowest NMED and a small size. Regarding accuracy, the designs based on \textit{InXA1} have low ER and NMED. Similarly, the designs based on the 6 transistors FA, have the minimal size. Thus, it can be observed that the characteristics of approximate FA are generally propagated in the corresponding approximate multipliers as well.

%Based on the above-mentioned design space exploration, we notice that approximate multipliers based on the InXA2 FA, exhibit the lowest ER and NMED, because this FA gives an exact value for the \textit{Cout} output, which significantly contributes toward the quality of the result. 

%Moreover, the designs based on InXA1 have the least delay and low ER. Similarly, the designs based on the 6 transistor FAs are generally found to be superior in their size. 

%Finally, the designs based on AMA5 generally have the lowest power consumption, and a low delay. 

In terms of architecture, we found that the tree multiplier designs tend to have a lower power consumption than array multipliers, especially the designs based on low power consumption FAs, such as \textit{AMA3} and \textit{AMA5}. In terms of the 8x8 sub-module placement to form higher-order multipliers, with a fixed configuration for AHxBH, AHxBL and ALxBH sub-module, we have noticed that ER and NMED increase, while the size, power consumption and delay decrease for designs with a high degree of approximation in ALxBL.

Compared to the 24 different designs reported in \cite{Jiang}, where 92\% of the designs have ER close to 100\%, only 80\% of our proposed designs have high ER. Regarding NMED, almost all our designs have a value less than 10\textsuperscript{-5}, which is the minimum value reported by the 24 approximate designs in \cite{Jiang}. Comparing the PDP reduction, most of the designs in \cite{Jiang} have a high PDP reduction because they are based on truncation and a high degree of approximation. However, our designs are superior in PDP reduction for designs with a high degree of approximation.

==> Arxiv-Online-Comparative-TR uploaded/Introduction.tex <==
\section{Introduction}
\label{introduction}
	The pervasive, portable, embedded and mobile nature of present age computing systems has led to an increasing demand for ultra low power consumption, small footprint, and high performance. Approximate computing \cite{AC1} is a nascent computing paradigm that allows us to achieve these objectives by compromising the arithmetic accuracy. Many systems used in domains, like multimedia and big data analysis, exhibit an inherent tolerance to a certain level of inaccuracies in computation, and thus can benefit from approximate computing.

Functional approximation \cite{M5}, in hardware, mostly deals with the design of approximate arithmetic units, such as adders and multipliers, at different abstraction levels, i.e., transistor, gate, RTL (Register Transfer Level) and application. Some notable approximate adders include \textit{speculative adders}\cite{speculative}, \textit{segmented adders}\cite{segmented}, \textit{carry select adders}\cite{CSA} and \textit{approximate full adders} \cite{AC2}. The transistor level approximation provides the highest flexibility due to the ability to tweak most of the design parameters at this level. Various approximate full adders (FA) at the transistor level have been proposed including the mirror adders \cite{Vaibhav}, the XOR/XNOR based FA \cite{XORFA} and the inexact FA \cite{InXA}. On the other hand, most of approximate multipliers have been designed at higher levels of abstraction, i.e., gate, RTL and application. 

Approximate multipliers have been mainly designed using three techniques, i) \textit{Approximation in partial products generation}: e.g., Kulkarni et al. \cite{M5} proposed an approximate 2x2 binary multiplier at the gate level by changing a single entry in the Karnaugh-map with an error rate of $1/16$. ii) \textit{Approximation in partial product tree}: e.g., Error Tolerant Multipliers (ETM) \cite{M6} divide the input operands in  two parts, i.e., the multiplication part for the MSBs and the non-multiplication part for the LSBs, and thus omitting the generation of some partial products \cite{M1}. iii) \textit{Approximation in partial products summation}: Approximate FA cells are used to form an array multiplier, e.g., in \cite{Reddy} the approximate mirror adder has been used to develop a multiplier. Similarly, Momeni et al. \cite{M2} proposed an approximate compressor for building approximate multipliers, but this multiplier is known to give a non-zero result for zero inputs. Jiang et al.\cite{Jiang} compared the characteristics of different approximate multipliers, implemented in VHDL based on the three different techniques mentioned previously. \textit{In this work, we target approximate multipliers based on approximation in partial products summation}.

In this report, we compare the accuracy and circuit characteristics of different approximate multipliers. These multipliers are designed based on three identified decisions: (1) the type of approximate FA used to construct the multiplier, (2) the architecture of the multiplier, and (3) the placement of sub-modules of approximate and exact multipliers in the target multiplier module. We were able to design  approximate multipliers, which are suitable to applications with intrinsic error resiliency. We used these designs in an image processing application and obtained promising results, thus we believe they are applicable in other domains. The rest of the report is organized as follows: The proposed methodology of designing and evaluating approximate multipliers is explained in Section \ref{methodology}. Section \ref{sec:ApproxFA} explains the design characteristics of approximate FAs and compressors. Section \ref{sec:8X8} describes different configurations of approximate sub-modules, with different architectures. Target approximate multiplies are designed and evaluated in Section \ref{sec:MainModule}. The application of image processing is given in Section \ref{sec:application}. Finally, conclusions are drawn in Section \ref{sec:conclusion}.


==> Arxiv-Online-Comparative-TR uploaded/Methodology.tex <==
\section{Proposed Methodology}
\label{methodology}

The design space for approximate multipliers based on different approximate FAs and compressors is quite huge. However, it is difficult to select the most suitable design for a specific application. Figure \ref{fig:methodology} presents an overview of our proposed methodology to build different approximate multipliers and compare their design metrics to select the most suitable design. It consists of the following steps:
%\includegraphics[width=9cm]{Methodology11.jpg}



%Therefore, there is a dire need for power-quality configurable approximate multipliers with high flexibility and reconfigurability
\begin{enumerate}
\item \textit{Building a library of elementary approximate FAs using the TSMC65nm technology in Cadence Spectre}: We use the default transistors of this technology to build 11 approximate FA designs comprising of 5 mirror FAs, 3 XOR/XNOR gate FAs and 3 inexact FAs. To the best of our knowledge, these 11 designs are the only ones that exist in the literature at the transistor level.
 
\item \textit{Characterization and early space reduction}: We perform area, power, latency and quality characterizations of different approximate FAs to filter out non-Pareto designs. %\textcolor{red}{In this work we didn't eliminate any FA to have more designs}.

\begin{figure}[h]
\centering
%
\includegraphics[width=1.0\textwidth, height=10cm]{m.png}
\centering
%\includegraphics[width=9cm]{method.png}
\caption{Methodology Overview}
\label{fig:methodology}
\end{figure}

\item \textit{Building a library of approximate compressors}: We build a Cadence library of approximate compressors using the optimal approximate FA, as recommended by \cite{Vaibhav}.

\item \textit{Building approximate multipliers basic blocks}: Based on approximate FAs and compressors, we design various approximate 8x8 array and tree multipliers, respectively. These proposed designs are related to the ripple-carry array multiplier architecture, which is the most power efficient amonge conventional architectures \cite{Mrazek}.
%in Cadence Spectre. These 8x8 multipliers are used as foundational blocks to design higher-order approximate multipliers.

\item \textit{Design target approximate multipliers}: Based on different configurations of 8x8 approximate multipliers, the target multiplier modules are designed and characterized.

\item \textit{Selection of design points}: Considering the required quality constrains of a specific application, a subset of power-efficient design points is selected.
\end{enumerate}

In order to evaluate the efficiency of the proposed approximate designs, \textit{power consumption} and \textit{area}, represented by the number of transistors used, are measured, and the circuit performance is measured by the maximum \textit{delay} between changing the inputs and observing the output(s). Besides these basic design metrics, \textit{accuracy} is also an important design constraint in approximate computing. There exist several \textit{error metrics} used in approximate computing to quantify errors and measure accuracy \cite{InXA}, including:
\begin{itemize}
\item Error Rate (ER): The percentage of erroneous outputs among all outputs.

\item Error Distance (ED): The arithmetic difference between the exact and approximate result.

\item Mean Error Distance (MED): The average of EDs for a set of outputs obtained by applying a set of inputs.

\item Relative Error Distance (RED): The ratio of ED to exact result. 
 
\item Mean Relative Error Distance (MRED): The average value of all possible relative error distances (RED).

\item Normalized Mean Error Distance (NMED): The normalization of mean error distance (MED) by the maximum output of the accurate design. This metric is used for comparing circuits (adders and multipliers) of different sizes. 

\end{itemize}
 %Error Rate (ER), Error Distance (ED), Mean Error Distance (MED), Normalized Mean Error Distance (NMED), Relative Error Distance (RED) and Mean Relative Error Distance (MRED). 
 
For the evaluation of the accuracy of the approximate FAs, we use the number of erroneous outputs. In the proposed methodology, we evaluate ER, MED, NMED and MRED for the proposed designs. As shown in Figure \ref{fig:methodology}, \textit{the characterization and selection} process is applied at multiple steps to different components, during the design flow. Characterization aims to find the design characteristics of the circuits including area, power consumption, performance, error metrics, and other derived metrics such as Power-Delay-Product (PDP). The design selection process for the evaluated approximate designs also depends on the application domain of the given circuit. As the design requirements vary from one application to another, our designs are unique because they can provide some degree of error in the output as well and thus this aspect also needs to be covered in the characterization and selection process.

%However ER is the basic accuracy metric, and NMED is used to comapre designs of different sizes.

==> Arxiv-Online-Comparative-TR uploaded/abstractnew.tex <==
\title{\Large{\textbf{Comparative Study of Approximate  Multipliers}}}
\author{
Mahmoud~Masadeh$^{1}$, Osman~Hasan$^{1,2}$, and Sofi\`ene~Tahar$^{1}$ \vspace*{2em}\\
$^{1}$Department of Electrical and Computer Engineering,\\
Concordia University, Montr\'eal, Canada  \\
\{m\_masa,o\_hasan,tahar\}@ece.concordia.ca \vspace*{2em}\\
$^{2}$School of Electrical Engineering and Computer Science,\\
National University of Science and Technology, Islamabad, Pakistan \\
\\
TECHNICAL REPORT \\
\date{March 2018}
}
\maketitle

\newpage
\begin{abstract}

%Approximate multipliers are widely being advocated for energy-efficient computing in applications that exhibit an inherent tolerance to inaccuracy. In this paper, we identify three decisions for design and evaluation of approximate multiplier circuits: (1) the type of approximate full adder (FA) used to construct the multiplier, (2) the architecture, i.e., array or tree, of the multiplier and (3) the placement of sub-modules of approximate and exact multipliers in the target multiplier module. Based on FA cells implemented at the transistor level (TSMC65nm), we developed several approximate building blocks of 8x8 multipliers, as well as various implementations of higher order multipliers. These designs are evaluated based on their power, area, delay and error and the best designs are identified. We validate these designs on an image blending application using MATLAB, and compare them to related work. The library of implemented cells and multiplier circuits is available as an open source.

Approximate multipliers are widely being advocated for energy-efficient computing in applications that exhibit an inherent tolerance to inaccuracy.  However, the inclusion of accuracy as a key design parameter, besides the performance, area and power, makes the identification of the most suitable approximate multiplier quite challenging. In this paper, we identify three major decision making factors for the selection of an approximate multipliers circuit: (1) the type of approximate full adder (FA) used to construct the multiplier, (2) the architecture, i.e., array or tree, of the multiplier and (3) the placement of sub-modules of approximate and exact multipliers in the main multiplier module. Based on these factors, we explored the design space for circuit level implementations of approximate multipliers. We used circuit level implementations of some of the most widely used approximate full adders, i.e., approximate mirror adders, XOR/XNOR based approximate full adders and Inexact adder cell. These FA cells are then used to develop circuits for the approximate high order compressors as building blocks for 8x8 array and tree multipliers. We then develop various implementations of higher bit multipliers by using a combination of exact and inaccurate 8x8 multiplier cells. All these implementations have been done using the Cadence's Spectre tool with the TSMC65nm technology. The design space of these multipliers is explored based on their power, area, delay and error and the best approximate multiplier designs are identified. The report also presents the validation of our results using an image blending application. An open source library of implemented cells and multiplier circuits are available online.
%at https://sourceforge.net/projects/approximatemultiplier.

\end{abstract}
\keywords{Approximate Computing, Approximate Multiplier, Power-Efficiency, Error Metrics, Circuit Characteristics,
Comparative Study}

\newpage
\tableofcontents
